PsybORG+: Modeling and Simulation for Detecting Cognitive Biases in Advanced Persistent Threats

Advanced Persistent Threats (APTs) bring significant challenges to cybersecurity due to their sophisticated and stealthy nature. Traditional cybersecurity measures fail to defend against APTs. Cognitive vulnerabilities can significantly influence attackers' decision-making processes, which presents an opportunity for defenders to exploit. This work introduces PsybORG$^+$, a multi-agent cybersecurity simulation environment designed to model APT behaviors influenced by cognitive vulnerabilities. A classification model is built for cognitive vulnerability inference and a simulator is designed for synthetic data generation. Results show that PsybORG$^+$ can effectively model APT attackers with different loss aversion and confirmation bias levels. The classification model has at least a 0.83 accuracy rate in predicting cognitive vulnerabilities.

==> trigger.tex <==
% In psychology, a trigger refers to a stimulus that can influence our psychological preferences to change our behavior\cite{matsumura2015shikakeology}. A notable instance is Post-Traumatic Stress Disorder (PTSD). Triggers like sounds and sights can prompt symptoms like flashbacks, anxiety, and hypervigilance in individuals with PTSD\cite{yehuda2015post}. 

A trigger is a system condition designed to provoke attackers into revealing their cognitive vulnerabilities. Triggers can take many forms, including deploying honeypots, creating fake files and accounts, and exposing simulated vulnerabilities. Setting up appropriate triggers is an effective strategy for detecting features of APTs.

\subsection{Sunk Cost Fallacy Trigger in PsybORG$^+$}
We can implement a trigger in PsybORG$^+$ to highlight the differences in actions among attackers with varying degrees of sunk cost fallacy. By placing a group of password-protected files with enticing filenames within the subnet and adding credential files on workstations, we create a trigger for the sunk cost fallacy. Some of these credential files are fake and useless for cracking the passwords, while the others are genuine and can significantly increase the success rate of cracking the passwords. Attackers exhibiting sunk cost fallacy are likely to invest considerable time and effort into cracking these passwords and testing the credential files once they find them.

\subsection{Evaluation of PsybORG$^+$ with Trigger}
We utilize the same dataset and settings as the experimental environment for synthetic data generation, with the addition of a trigger in PsybORG$^+$. Initially, a group of high-value, high-difficulty files is created on the host. In the 200th step, numerous credential files containing filename-password mappings are placed on server\_host\_0 of each subnet, with 20\% of these credential files being fake.

This setup results in a significant increase in the decision tree's classification accuracy rate for detecting sunk cost fallacy, rising from 0.4 to 0.83. The classification results of the new model are illustrated in Figure \ref{decision_tree_trigger}.


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/dt_4_trigger_vertical.png}
    \caption{Data-driven Decision Tree with trigger}
    \label{decision_tree_trigger}
\end{figure}

We also compare our simulator with the two baselines mentioned earlier in this new environment. As shown in Figure \ref{compare3} and Table \ref{dis2}, there is a significant difference between our simulator's results and the simulation results with random parameters regarding maximum cracking attempts in most bias states. This indicates that the trigger successfully induces attackers to exhibit varying degrees of sunk cost fallacy. The small distance between the synthetic data generated by our simulator and the synthetic data generated by attackers using real parameters to mimic the inputted data demonstrates our simulator's excellent performance.

\begin{figure}[htb] 
	\centering  
	%\vspace{-0.35cm}
	\subfigtopskip=2pt
	\subfigbottomskip=2pt 
	\subfigcapskip=-5pt
	\subfigure[Rate of doing aggressive service discovery]{
		\label{aggressive_distance}
		\includegraphics[width=0.9\linewidth]{figures/ag_dis_4_trigger.png}}
\\
	\subfigure[Rate of doing confirming credential file checking]{
		\label{confirm_distribution}
		\includegraphics[width=0.9\linewidth]{figures/confirming evidence_trigger.png}}
\\
        \subfigure[Maximum attempts of cracking file on the same file]{
		\label{sunk_cost_fallacy_distribution}
		\includegraphics[width=0.9\linewidth]{figures/sunk_distance_trigger.png}}
	\caption{Evaluation of synthetic data (with trigger)}
	\label{compare3}
\end{figure}

\begin{table}[ht]
    \centering
    \caption{Distance between synthetic data and real data (with trigger)\label{dis2}}
    \begin{tabular}{ccccccc}
        \toprule
        &\multicolumn{1}{c}{Biases} & \multicolumn{1}{c}{Sampled parameter} & \multicolumn{1}{c}{Real parameter} &\multicolumn{1}{c}{Random parameter} \\
        \midrule
\multirow{8}{*}{\rotatebox{90}{\textbf{Service discovery}}}
        & $\theta_0$ & 0.09 $\pm$ 0.05 & 0.07 $\pm$ 0.05 & 0.20 $\pm$ 0.13 \\
        & $\theta_1$ & 0.07 $\pm$ 0.05 & 0.06 $\pm$ 0.04 & 0.20 $\pm$ 0.14 \\
        & $\theta_2$ & 0.08 $\pm$ 0.05 & 0.06 $\pm$ 0.04 & 0.24 $\pm$ 0.14 \\
        & $\theta_3$ & 0.09 $\pm$ 0.06 & 0.06 $\pm$ 0.04 & 0.18 $\pm$ 0.15 \\
        & $\theta_4$ & 0.09 $\pm$ 0.06 & 0.07 $\pm$ 0.05 & 0.19 $\pm$ 0.16 \\
        & $\theta_5$ & 0.10 $\pm$ 0.07 & 0.06 $\pm$ 0.04 & 0.20 $\pm$ 0.17 \\
        & $\theta_6$ & 0.08 $\pm$ 0.06 & 0.05 $\pm$ 0.04 & 0.21 $\pm$ 0.15 \\
        & $\theta_7$ & 0.09 $\pm$ 0.07 & 0.07 $\pm$ 0.06 & 0.20 $\pm$ 0.15 \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{\textbf{Cred file checking}}}
        & $\theta_0$ & 0.13 $\pm$ 0.10 & 0.04 $\pm$ 0.05 & 0.41 $\pm$ 0.25 \\
        & $\theta_1$ & 0.13 $\pm$ 0.11 & 0.04 $\pm$ 0.04 & 0.36 $\pm$ 0.27 \\
        & $\theta_2$ & 0.14 $\pm$ 0.10 & 0.04 $\pm$ 0.04 & 0.36 $\pm$ 0.22 \\
        & $\theta_3$ & 0.14 $\pm$ 0.08 & 0.05 $\pm$ 0.04 & 0.39 $\pm$ 0.23 \\
        & $\theta_4$ & 0.13 $\pm$ 0.10 & 0.05 $\pm$ 0.04 & 0.36 $\pm$ 0.23 \\
        & $\theta_5$ & 0.13 $\pm$ 0.10 & 0.05 $\pm$ 0.04 & 0.34 $\pm$ 0.23 \\
        & $\theta_6$ & 0.10 $\pm$ 0.08 & 0.04 $\pm$ 0.04 & 0.40 $\pm$ 0.27 \\
        & $\theta_7$ & 0.13 $\pm$ 0.11 & 0.05 $\pm$ 0.04 & 0.38 $\pm$ 0.26 \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{\textbf{File cracking}}}
        & $\theta_0$ & 2.14 $\pm$ 2.10 & 2.30 $\pm$ 1.71 & 3.18 $\pm$ 2.61 \\
        & $\theta_1$ & 3.60 $\pm$ 3.41 & 3.22 $\pm$ 2.64 & 3.34 $\pm$ 2.57 \\
        & $\theta_2$ & 2.68 $\pm$ 2.27 & 2.44 $\pm$ 2.01 & 3.34 $\pm$ 2.70 \\
        & $\theta_3$ & 3.14 $\pm$ 2.89 & 3.36 $\pm$ 3.12 & 4.30 $\pm$ 3.60 \\
        & $\theta_4$ & 2.36 $\pm$ 2.11 & 2.42 $\pm$ 1.86 & 3.24 $\pm$ 2.53 \\
        & $\theta_5$ & 3.32 $\pm$ 3.29 & 3.34 $\pm$ 3.15 & 4.44 $\pm$ 3.26 \\
        & $\theta_6$ & 2.24 $\pm$ 2.45 & 2.08 $\pm$ 1.43 & 3.54 $\pm$ 2.57 \\
        & $\theta_7$ & 3.10 $\pm$ 2.87 & 3.04 $\pm$ 2.44 & 3.22 $\pm$ 2.27 \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Hypothesis test on trigger}
To further evaluate the effectiveness of our trigger, we perform a hypothesis test on the maximum cracking attempts of all high sunk cost fallacy attackers' simulation results in PsybORG$^+$ with the trigger ($w$) and PsybORG$^+$ without the trigger ($w'$). 

% At first, we apply the Shapiro-Wilk test\cite{razali2011power} on the distributions of max cracking times in $w$ and $w'$. The result shows that both distributions follow the normal distribution.

% , as presented in Table \ref{sw_test}. 

We conduct a T-test\cite{dienes2014using} where we select $w'$ as the control group and $w$ as the experimental group. Our null hypothesis is that the trigger has no significant effect on the number of cracking attempts. The results are as follows: $T$-statistic $= 40.38$ and $P$-value $= 7.81e-143$. Given the extremely small $p$-value, we rejected the null hypothesis.

% \begin{table}[!h]
% \centering
% \caption{\label{sw_test}Shapiro-Wilk test result}
% \begin{tabular}{|c|c|c|}
% 	\hline data&statistic&pvalue\\
%         \hline $w$&0.93&0 \\
%         \hline $w'$&0.84&0 \\
%     \hline
% \end{tabular}
% \end{table}
